Unbiased Graph Embedding with Biased Graph Observations

Graph embedding techniques are pivotal in real-world machine learning tasks that operate on graph-structured data, such as social recommendation and protein structure modeling. Embeddings are mostly performed on the node level for learning representations of each node. Since the formation of a graph is inevitably affected by certain sensitive node attributes, the node embeddings can inherit such sensitive information and introduce undesirable biases in downstream tasks. Most existing works impose ad-hoc constraints on the node embeddings to restrict their distributions for unbiasedness/fairness, which however compromise the utility of the resulting embeddings. In this paper, we propose a principled new way for unbiased graph embedding by learning node embeddings from an underlying bias-free graph, which is not influenced by sensitive node attributes. Motivated by this new perspective, we propose two complementary methods for uncovering such an underlying graph, with the goal of introducing minimum impact on the utility of the embeddings. Both our theoretical justification and extensive experimental comparisons against state-of-the-art solutions demonstrate the effectiveness of our proposed methods.

==> method_backup.tex <==
\section{Preliminaries}
\label{sec:preliminary}
In this section, we first introduce our notations and general graph embedding concepts. Then we discuss the criterion under which we evaluate if the graph embeddings are (un)biased. 

\subsection{Notations}
Let $\gG = (\gV, \gE, \gA)$ be an undirected, attributed graph with a set of $N$ nodes $\gV$, a set of edges $\gE \subseteq \gV\times\gV$, and a set of $N$ attribute vectors $\gA$ (one attribute vector for each node). We use $(u,v)$ to denote an edge between node $u\in\gV$ and node $v\in\gV$. The number of attributes on each node is $K$, and $\gA = \{\va_1, \va_2, \dots, \va_n\}$, where $\va_u$ is an $K$-dimensional attribute vector for node $u$. We assume that all attributes are categorical and $\gS_i$ is the set of all possible values for attribute $i$. For example, if node $u$ is a person node, and the $i$-th attribute is gender with possible values $\gS_i=\{0,1\}$, then $\va_u[i]=0$ indicates that $u$ is a female. 
% Without loss of generality, we assume the first $m$ attributes are sensitive attributes, and the values for the rest of attributes is represented by $\va_u[m:]$ for node $u$, where we follow Python's indexing style to slice a vector. 
% We first focus on the case of single sensitive attribute and $m=1$.

We focus on the link prediction task in this paper. In the problem of graph embedding learning, we aim to learn an encoder $\mathrm{ENC}:\gV\rightarrow\sR^d$ that maps each node $u$ to a $d$-dimensional embedding vector $\vz_u=\mathrm{ENC}(u)$. There is a scoring function $\rs(\vz_u, \vz_v)$ which predicts the probability of an edge between node $u$ and node $v$ in the given graph, i.e., $(u,v)\in\gE$. The loss for learning the embeddings and possible parameters for the scoring function are defined by:
\begin{equation}
\label{eq:loss}
    \sum_{(u,v)\in\gE} \gL_{edge}(\rs(\vz_u, \vz_v)),
\end{equation}
where $\gL_{edge}$ is a per-edge loss function on $(u,v)\in\gE$. Such loss functions generally aim to maximize the likelihood of observed edges between node pairs in the given graph, comparing to the negative samples of node pairs where edges are not observed.

\subsection{Unbiased Graph Embeddings}
Since the bias/fairness issues emerge most notably in prediction tasks involving humans, such as loan application \cite{kulik2000demographics} or criminal justice \cite{berk2021fairness}, we will use user-related graphs as examples to discuss our criterion for unbiased graph embeddings. And to simplify our discussion, we assume the attribute vector $\va_u$ only contains sensitive attributes that need to be debiased. But we have to emphasize this setting is only to illustrate the concept of biased graph embeddings; and our proposed solution can be applied to any graph data to remove biases caused by pre-defined sensitive attributes in the learnt embeddings.

Given a user node $u$, we consider its embedding $\vz_u$ is unbiased if it is independent from the sensitive attributes $\va_u$,
\begin{equation}
    \vz_u \perp \va_u, \forall u\in\gV. 
\end{equation}
% Should this holds for each attribute independently as in compositional fairness or this should hold for the whole attribute vector? 
This is equivalent to saying that the mutual information between $\vz_u$ and $\va_u$ is $\mathrm I(\vz_u, \va_u)=0$. This formulation of unbiasedness is similar to \citet{bose2019compositional}, but we consider the unbiasedness on the combination of all sensitive attributes, instead of on each sensitive attribute independently. %and can be easily generalized to the case of multiple sensitive attributes. 

Prior work measures such  unbiasedness in the learnt embeddings by their quality in predicting the value of the sensitive attributes \cite{palowitch2020monet,buyl2020debayes}. For example, we can evaluate the unbiasedness of learnt embeddings by training a classifier on a subset of user nodes' embeddings and their sensitive attributes. If the classifier cannot predict the sensitive attribute values of other user nodes, we claim that the embeddings have low bias. If the prediction accuracy equals to that from random embeddings, the user embeddings is considered bias-free. In fact, such classifier is often used as the discriminator in algorithmic methods where the classifier and the embeddings are learnt jointly: the embeddings are pushed to directions where the classifier has low prediction accuracy. 

% fairness measures
There are also studies that use fairness measures such as demographic parity or equalized opportunity to define the unbiasedness of learnt embeddings \cite{hardt2016equality,buyl2020debayes}. But we should point out that such fairness measures can only evaluate the fairness of the final prediction results for the intended downstream tasks, but cannot assess whether the embeddings are biased by, or contain any information about, sensitive attributes. In particular, fairness in a downstream task is only a necessary condition for unbiased embedding learning, not sufficient. The logic is obvious: unbiased embeddings can lead to fair prediction results as no sensitive attribute information is involved; but obtaining fairness in one task does not suggest the embeddings themselves are fair, e.g., those embeddings can still have unfair results in other tasks or even the fair results are obtained by other means, such as post-processing of the prediction results \citet{woodworth2017learning}. 
In \Cref{sec:exp}, we will use both the prediction accuracy on sensitive attribute values and fairness measures on final prediction results to evaluate the performance of our unbiased graph embedding. 

\section{Effect of attributes in graph generation}
\label{sec:under-graph}
In this section, we discuss the generation of an observed graph by explicitly modeling the effects of user attributes in the procedure, which will help us debias such effect. In particular, we assume that there is an underlying graph whose edge distribution is decided by global graph properties and node features not included in $\va_u$, such as the degree distributions. Then the user attributes will modify the edge distribution of the underlying graph based on effects like \emph{homophily} in social networks, where links are created based on the attribute similarities of the individuals \cite{mcpherson2001birds,fond2010randomization}. The new distribution is then used to generate the observed graph. 

Formally, let $\gM$ be a generative graph model and $\Theta_{M}$ be the set of parameters that describe the global properties of the underlying graph. We consider the class of generative graph models that represent the set of possible edges in the graph as binary random variables $E_{uv},u\in\gV,v\in\gV$. In this case the event $E_{uv}=1$ implies $(u,v)\in\gE$ (and $(v,u)\in\gE$ in undirected graphs). The model $\gM$ assigns a probability to $E_{uv}$ based on $\Theta_{M}$, $P_M(E_{uv}=1|\Theta_M)$. Therefore, the edge set $\gE$ can be considered as drawn by sampling each edge according to $Bernoulli(P_M(E_{uv}=1|\Theta_M)), \forall u\in\gV, \forall v\in\gV$. There are many such models $\gM$ such as the Chung Lu model \cite{Chung2002average} and Kronecker Product Graph Model \cite{leskovec2010kronecker}. Note that $\gM$ does not consider user attributes $\gA$ in the generation of the graph.  

Now we involve the user attributes in the generation of a graph. Specifically, let $C_{uv}\in\gA\times\gA$ be a random variable indicating the attribute value combination between $u$ and $v$, which is independent from $\Theta_M$. $P_{o}(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ is the conditional distribution of an edge in the observed graph given the corresponding attributes on the incident nodes and the global parameters $\Theta_M$, where $\va_{uv}= (\va_u, \va_v)$ represents the combination of attribute values from the two incident nodes $u$ and $v$. Note that there can be many node pairs that have the same attribute value combination. Based on Bayes' Theorem, we have 
\begin{align}
\label{eq:bayes}
    & P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)  \\\nonumber
   =\,& \frac{P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)P_o(E_{uv}=1|\Theta_M)}{P_o(C_{uv}=\va_{uv}|\Theta_M)} \\\nonumber
   =\,& P_M(E_{uv}=1|\Theta_M)\frac{P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)}{P_o(C_{uv}=\va_{uv}|\Theta_M)},\forall u\in\gV, \forall v\in\gV,
\end{align}
where we assume the prior distribution on $E_{uv}$ is defined by an underlying model $\gM$, $P_o(E_{uv}=1|\Theta_M) = P_M(E_{uv}=1|\Theta_M)$, and the posterior distribution accounts for the specific attribute value combinations. Therefore, the edge distribution of the observed graph with node attributes is a modification of the underlying graph distribution defined by $\gM$ and $\Theta_M$. It is important to note that we do not need to include all possible characteristics of a node $u$ in $\va_{u}$. In fact, some characteristics can be treated as node features captured by $\Theta_M$ used by $\gM$ in generating the underlying graph. Thus we only need to include attributes whose effect is under our interests in $\va_{u}$. For instance, $\va_u$ can include sensitive attributes we want to debias. It can also include attributes that could correlate with the sensitive attributes whose effects are meant to be explicitly kept from the influence of debiasing the sensitive attribute for better utility. 

Let us define a function that maps the attribute value combinations $\va_{uv}$ to the probability ratio that modifies the underlying graph into the observed graph by
\begin{equation}
    R(\va_{uv}) \coloneqq \frac{P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)}{P_o(C_{uv}=\va_{uv}|\Theta_M)}, \forall u\in\gV, \forall v\in\gV.
\end{equation}
Thus we can rewrite \Eqref{eq:bayes} by 
\begin{equation}
\label{eq:prob-decomp}
    P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M) = P_M(E_{uv}=1|\Theta_M)R(\va_{uv}). 
\end{equation}
In this way, we explicitly model the effect of node attributes by $R(\va_{uv})$, which modifies the underlying graph distribution $P_M(E_{uv}=1|\Theta_M)R(\va_{uv})$ for generating the given observed graph $\gG$. 

\section{Unbiased Graph Embedding from a Bias-Free Graph}
\label{sec:UGE}
In this section, we propose methods for learning unbiased node embeddings that are independent from sensitive attributes, based on the understanding of their effects in \Cref{sec:under-graph}. Without loss of generality, we assume the first $m$ attributes are sensitive attributes, and the values for the rest of attributes is represented by $\va_u[m:]$ for node $u$. Now consider a world without the sensitive attributes, and the attribute vector of node $u$ becomes $\tilde\va_u = \va_u[m:]$. We denote by $\tilde{\gG}=(\gV, \tilde\gE, \tilde\gA)$ a new graph generated with $\tilde\va_u, \forall u\in\gV$. Therefore, if we can learn the node embeddings from $\tilde\gG$ instead of $\gG$, the embeddings are guaranteed to be unbiased with respect to sensitive attributes. Specifically, the edge probabilities in $\tilde\gG$ can be written as
\begin{equation}
\label{eq:prob-decomp2}
    P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M) = P_M(E_{uv}=1|\Theta_M)\tilde R(\tilde\va_{uv}), 
\end{equation}
where
\begin{equation}
    \tilde R(\tilde\va_{uv}) \coloneqq \frac{P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M)}{P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|\Theta_M)}, \forall u\in\gV, \forall v\in\gV,
\end{equation}
$\tilde{C}_{uv}$ is the random variable indicating attribute value combinations without sensitive attributes, and $P_{\tilde o}$ indicates the distributions used in generating $\tilde\gG$. We call the class of methods that learn embeddings from $\tilde\gG$ unbiased graph embedding, or \UGE in short. Next we discuss two instance of \UGE. The first method is called \UGE-W, which reweighs the per-edge loss such that the total loss is from $\gG$ in expectation. The second method is called \UGE-R, which adds an regularization term to push the embeddings to be equivalent as directly learnt from $\tilde\gG$.

\subsection{Weighting Based \UGE}
We modify the loss function in \Eqref{eq:loss} by reweighing each loss term on an edge as
\begin{equation}
\label{eq:ube-loss}
    \gL_{\UGE-W}(\gG) = \sum_{(u,v)\in\gE} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})}.
\end{equation}
\begin{theorem}
Given a graph $\gG$, and the ratio $\tilde R(\tilde\va_{uv}) / R(\va_{uv}), \forall (u,v)\in\gE$,  $\gL_{\UGE-W}(\gG)$ is an unbiased loss with respect to $\tilde\gG$.
\end{theorem}
\begin{proof}
\begin{align}
\label{eq:expectation}
    & \E\big[\gL_{\UGE-W}(\gG)\big] \\\nonumber
    =\,& \E\Bigg[\sum_{(u,v)\in\gE} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})}\Bigg] \\\nonumber
    =\,& \E\Bigg[\sum_{u\in\gV, v\in\gV} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})}\cdot E_{uv}\Bigg] \\\nonumber
    =\,& \sum_{u\in\gV, v\in\gV} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})} \cdot P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M) \\\nonumber  
    *=\,& \sum_{u\in\gV, v\in\gV} \gL_{edge}(\rs(\vz_u, \vz_v))\cdot P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M) \\\nonumber
    =\,& \E\Bigg[\sum_{(u,v)\in\tilde\gE} \gL_{edge}(\rs(\vz_u, \vz_v))\Bigg].
\end{align}
The step marked with $*$ uses \Eqref{eq:prob-decomp} and \Eqref{eq:prob-decomp2}.
\end{proof}
\noindent Therefore, we show that \Eqref{eq:ube-loss} is an unbiased loss on the new graph $\tilde\gG$. Since $\UGE-W$ is learning node embeddings from a graph where no sensitive attribute is present, it is sufficient for the embeddings to be unbiased. 

The only thing needed for deploying \UGE-W in existing graph embedding methods is the weights $\tilde R(\tilde\va_{uv})/R(\va_{uv})$. 
% relation to importance sampling, observational study, unbiased l2r
Now we discuss the estimation of $R(\va_{uv})$ and $\tilde R(\va_{uv})$. For estimating $R(\va_{uv})$, we need estimates for two probabilities $P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)$ and $P_o(C_{uv}=\va_{uv}|\Theta_M)$. With maximum likelihood estimates, we have 
\begin{align}
\label{eq:estimate-R}
    P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M) &\approx \frac{\sum_{(i,j)\in\gE}\sI[\va_{ij}=\va_{uv}]}{|\gE|}, \\
    P_o(C_{uv}=\va_{uv}|\Theta_M) &\approx \frac{\sum_{i\in\gV,j\in\gV}\sI[\va_{ij}=\va_{uv}]}{N^2}.
\end{align}
Similarly we can estimate $\tilde R(\tilde \va_{uv})$ by
\begin{align}
    P_o(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M) &\approx \frac{\sum_{(i,j)\in\tilde\gE}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{|\tilde\gE|}, \\\label{eq:estimate-tildeR}
    P_o(\tilde{C}_{uv}=\tilde\va_{uv}|\Theta_M) &\approx \frac{\sum_{i\in\gV,j\in\gV}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{N^2}.
\end{align}
Note that the estimation of $P_o(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M)$ is based on $\tilde\gE$, which is not directly observable. However, we show that we can estimate $P_o(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M)$ with $\gE$ with the following assumption: after grouping node pairs by non-sensitive attribute value combinations $\tilde\va_{uv}$, the sensitive attributes only re-route the edges while do not change the number of edges in each group. Then we have
\begin{align}
    P_o(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M) &\approx \frac{\sum_{(i,j)\in\tilde\gE}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{|\tilde\gE|}, \\\nonumber
    &= \frac{\sum_{i\in\gV,j\in\gV,\tilde\va_{ij}=\tilde\va_{uv}}\sI[(i,j)\in\tilde\gE]}{|\tilde\gE|}, \\\nonumber
    &= \frac{\sum_{i\in\gV,j\in\gV,\tilde\va_{ij}=\tilde\va_{uv}}\sI[(i,j)\in\gE]}{|\tilde\gE|}, \\\nonumber
    &= \frac{\sum_{(i,j)\in\gE}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{|\gE|}.
\end{align}
Note that for node pairs with the same attribute value combination, \Eqref{eq:estimate-R}-\ref{eq:estimate-tildeR} only need to be calculated once instead of for each pair. This can be done by first grouping the node pairs by their attribute value combination and then perform estimation in each group.
% the assumption in estimating $\tilde R(\tilde \va_{uv})$; we may need to assume \Theta_M does not influence attribute combinations
% independence assumption when there are many attributes
% extend to other models for estimating the weights; take perspectives from social influence and homophily for estimating the probabilities

\subsection{Regularization Based \UGE}
We propose an alternative way for unbiased graph embedding which adds a regularization to the loss function that pushes the embeddings to the direction of representing the underlying graph $\tilde\gG$. Intuitively, if the node embeddings can produce the same edge probabilities with and without the sensitive attributes, we claim that they are unbiased to the sensitive attributes. To enforce this condition, we need to shrink the distance between $P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ and $P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M)$ estimated from node embeddings. Specifically, we can use the scores $\rs(\vz_u, \vz_v)$ as a proxy to represent the relative probability of an edge between $u$ and $v$, i.e., high $\rs(\vz_u, \vz_v)$ indicates high probability of an edge between $u$ and $v$. 
Since the probability $P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ of an edge conditioned on the node attribute value combination $\va_{uv}$
is the same for node pairs with the same attribute value combinations, we can estimate it by
\begin{align}
    & P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M) \\\nonumber 
    \approx&\; \frac{1}{T_{\va_{uv}}}\sum_{i\in\gV,j\in\gV,\va_{ij}=\va_{uv}}\rs(\vz_i, \vz_j) = Q_{\va_{uv}},
\end{align}
where we use $Q_{\va_{uv}}$ to denote the approximation, and $T_{\va_{uv}}$ is the number of pairs that has the attribute combination $\va_{uv}$. For node pairs with the same attribute value combination, $Q_{\va_{uv}}$ only need to be calculated once. $Q_{\tilde\va_{uv}}\approx P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M)$ can be obtained similarly from the embeddings, where $\tilde\va_{uv}$ is the same attribute value combination as $\va_{uv}$ with the sensitive attributes removed. Finally, we use $\ell_2$ distance between $Q_{\va_{uv}}$ and $Q_{\tilde\va_{uv}}$ for the regularization in the loss function
\begin{align}
    &\gL_{\UGE-R}(\gG) \\\nonumber
    =&\; \sum_{(u,v)\in\gE} \gL_{edge}(\rs(\vz_u, \vz_v)) + \lambda\sum_{u\in\gV, v\in\gV}\norm{Q_{\va_{uv}} - Q_{\tilde\va_{uv}}}_2,
\end{align}
where $\lambda$ controls the trade-off between the per-edge loss and the regularization.


\subsection{Discussion}
\label{sec:discuss-uge}
% relation to importance sampling, observational study, unbiased l2r
\UGE-W is similar to the idea of importance sampling \cite{kloek1978bayesian}, which analyze a particular distribution from the sample of a different distribution that is easy to sample from. In unbiased graph embedding, we aim to analyze the underlying graph $\tilde\gG$ by observations from the given graph $\gG$. Besides, in the estimation of $R(\tilde\va_{uv})/R(\va_{uv})$ and $R(\tilde\va_{uv})$ in \Eqref{eq:estimate-R} - \ref{eq:estimate-tildeR}, we group nodes by the combination of attribute values. However, when there are many attributes, the estimates may become inaccurate since each group only has a few nodes. In this case, we can further assume independence among the attributes, and thus the estimate for attribute combinations is the product of estimates for each attribute.

In contrast to adversarial regularizers,
\UGE-R is a different kind of regularization from the perspective of regularizing the distance between graphs with and without sensitive attributes recovered by the embeddings. The regularization term is summed over all node pairs, which can be costly. But in real implementations, we can add the regulariztaion by sampling node pairs in each iteration, and use $\lambda$ to control the strength of the regularization.

As mentioned, \UGE-W is a sufficient condition for unbiased node embeddings and \UGE-R is a necessary condition. We can combine them to trade-off the debiasing performance and utility,
\begin{align}
    &\gL_{\UGE-C}(\gG) \\\nonumber
    =&\; \sum_{(u,v)\in\gE} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})} + \lambda\sum_{u\in\gV, v\in\gV}\norm{Q_{\va_{uv}} - Q_{\tilde\va_{uv}}}_2,
\end{align}
where we use $\gL_{\UGE-C}(\gG)$ to represent the combined method. 

==> method_old_notation.tex <==
\section{Preliminaries}
\label{sec:preliminary}
In this section, we first introduce our notations and general graph embedding concepts. 
%Then we discuss the criterion under which we evaluate if the graph embeddings are unbiased. 
Since the bias/fairness issues emerge most notably in prediction tasks involving humans, such as loan application or job recommendation, we will use user-related graphs as running examples to discuss our criterion for unbiased graph embedding. But we have to emphasize that this setting is only to illustrate the concept of unbiased graph embedding; and our proposed solution can be applied to any graph data and selected sensitive attributes to avoid biases in the learned embeddings.

\subsection{Notation}
Let $\gG = (\gV, \gE, \gA)$ be an undirected, attributed graph with a set of $N$ nodes $\gV$, a set of edges $\gE \subseteq \gV\times\gV$, and a set of $N$ attribute vectors $\gA$ (one attribute vector for each node). We use $(u,v)$ to denote an edge between node $u$ and node $v$. The number of attributes on each node is $K$, and $\gA = \{\va_1, \va_2, \dots, \va_N\}$, where $\va_u$ is a $K$-dimensional attribute value vector for node $u$. %To simplify our discussion, we assume the attribute vector $\va_u$ only contains sensitive attributes that need to be debiased.
We assume all attributes are categorical and $\gS_i$ is the set of all possible values for attribute $i$. \footnote{We acknowledge that there are cases where attribute values are continuous, where discretization techniques can be applied.} For example, if node $u$ is a user node, and the $i$-th attribute is gender with possible values $\gS_i=\{\textit{Female},\textit{Male},\textit{Unknown}\}$, then $\va_u[i]=\textit{Female}$ indicates $u$ is a female. 
Without loss of generality, we assume the first $m$ attributes are sensitive, and $a_u[:m]$ and $a_u[m:]$ stands for the $m$ sensitive attributes and the rest of the attributes that are non-sensitive, respectively.

% Without loss of generality, we assume the first $m$ attributes are sensitive attributes, and the values for the rest of attributes is represented by $\va_u[m:]$ for node $u$, where we follow Python's indexing style to slice a vector. 
% We first focus on the case of single sensitive attribute and $m=1$.

In the problem of graph embedding learning, we aim to learn an encoder $\mathrm{ENC}:\gV\rightarrow\sR^d$ that maps each node $u$ to a $d$-dimensional embedding vector $\vz_u=\mathrm{ENC}(u)$. We focus on the \textit{unsupervised} embedding setting which does not require node labels and the embeddings are learned via the \textit{link prediction task}. In this task, a scoring function $\rs_{\btheta}(\vz_u, \vz_v)$ with parameters $\btheta$ is defined to predict the probability of an edge $(u,v)\in\gE$ between node $u$ and node $v$ in the given graph. The loss for learning node embeddings and parameters of the encoder and scoring function is defined by:
\begin{equation}
\label{eq:loss}
    \sum_{(u,v)\in\gE} \gL_{edge}(\rs_{\btheta}(\vz_u, \vz_v)),
\end{equation}
where $\gL_{edge}$ is a per-edge loss function on $(u,v)\in\gE$. Such loss functions generally aim to maximize the likelihood of observed edges in the given graph, comparing to the negative samples of node pairs where edges are not observed \cite{mikolov2013distributed,grover2016node2vec}.

\subsection{Unbiased Graph Embedding}
\label{sec:unbiased}
Given a node $u$, we consider its embedding $\vz_u$ as unbiased with respect to an attribute $i$ if it is independent from the attribute.
% , $\vz_u \perp \va_u[i], u\in\gV$.
% Should this holds for each attribute independently as in compositional fairness or this should hold for the whole attribute vector? 
% This is equivalent to require zero mutual information between $\vz_u$ and $\va_u[:m]$: i.e., $\mathrm I(\vz_u, \va_u[:m])=0$  \cite{bose2019compositional}.
Prior works evaluate such unbiasedness in the learned node embeddings by their ability to predict the values of the sensitive attributes \cite{bose2019compositional,palowitch2020monet,buyl2020debayes}. For example, they first train a classifier on a subset of node embeddings using their associated sensitive attribute values as labels. If the classifier cannot correctly predict the sensitive attribute values on the rest of node embeddings, one claims that the embeddings have low bias. If the prediction performance equals to that from random node embeddings, the learned embeddings are considered bias-free. In fact, such classifiers are often used as discriminators in adversarial methods where the classifier and the embeddings are learned jointly: the embeddings are pushed in directions where the classifier has low prediction accuracy \cite{madras2018learning,bose2019compositional}. 

% fairness measures
There are also studies that use fairness measures such as demographic parity or equalized opportunity to define the unbiasedness of learned embeddings \cite{hardt2016equality,buyl2020debayes}. But we need to clarify that such fairness measures can only evaluate the fairness of the final prediction results for the intended downstream tasks, but cannot assess whether the embeddings are biased by, or contain any information about, sensitive attributes. In particular, fairness in a downstream task is only a necessary condition for unbiased embedding learning, not sufficient. The logic is obvious: unbiased embeddings can lead to fair prediction results as no sensitive attribute information is involved; but obtaining fairness in one task does not suggest the embeddings themselves are unbiased, e.g., those embeddings can still lead to unfair results in other tasks or even the fair results are obtained by other means, such as post-processing of the prediction results \cite{woodworth2017learning}. 
In \Cref{sec:exp}, we will use both the prediction accuracy on sensitive attributes and fairness measures on final tasks to evaluate the effectiveness of our unbiased graph embedding methods. 

\section{Effect of attributes in graph generation}
\label{sec:under-graph}
In this section, we discuss the generation of an observed graph by explicitly modeling the effects of node attributes in the process. In particular, we assume that there is an \emph{underlying structural graph} behind an observed graph, whose edge distribution is governed by the global graph structural properties such as degree distributions, diameter, and clustering coefficients.
% , as well as node features, such as hobbies and public information of a user that are not demographic related or not included in a node's attribute vector\footnote{Such features are not considered as attributes and we are not interested in debiasing their impact in graph generation; and thus we include them as part of the underlying graph.}. 
The attributes in $\gA$ will modify the structural edge distribution based on effects like \emph{homophily} in social networks, where links are rewired based on the attribute similarities of the individuals \cite{mcpherson2001birds,fond2010randomization}. The modified edge distribution is then used to generate the observed graph. 

Formally, let $\gM$ be a structural generative graph model and $\Theta_{M}$ be the set of parameters that describe properties of the underlying structural graph. In particular, this set of parameters $\Theta_M$ is independent from node attributes in $\gA$. We consider the class of models that represent the set of possible edges in the graph as binary random variables $E_{uv},u\in\gV,v\in\gV$: i.e., the event $E_{uv}=1$ indicates $(u,v)\in\gE$. The model $\gM$ assigns a probability to $E_{uv}$ based on $\Theta_{M}$, $P_M(E_{uv}=1|\Theta_M)$. Therefore, the edges of an underlying structural graph $\gG_M$ can be considered as samples from $Bernoulli(P_M(E_{uv}=1|\Theta_M))$. There are many such structural models $\gM$ such as the Chung Lu model \cite{Chung2002average} and Kronecker Product Graph Model \cite{leskovec2010kronecker}. Note that $\gM$ does not consider node attributes in the generation of the structural graph.  

Now we involve the attributes in the generative process. Let $C_{uv}\in\{(\va_i,\va_j)|i\in\gV,j\in\gV\}$ be a random variable indicating the \emph{attribute value combination} of a randomly sampled pair of nodes $u$ and $v$, which is independent from $\Theta_M$. Note that $C_{uv}$ instantiated by different node pairs can be the same, as different nodes can have the same attribute values. $P_{o}(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ is the conditional probability of an edge $(u,v)$ given the corresponding attribute values on the incident nodes and structural parameters $\Theta_M$, where $\va_{uv}=(\va_u, \va_v)$ denotes the \emph{observed} attribute value combination on nodes $u$ and $v$. Based on Bayes' Theorem, we have
\begin{align}
\label{eq:bayes}
    & P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)  \\\nonumber
  =\,& \frac{P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)P_o(E_{uv}=1|\Theta_M)}{P_o(C_{uv}=\va_{uv}|\Theta_M)} \\\nonumber
  =\,& P_M(E_{uv}=1|\Theta_M)\frac{P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)}{P_o(C_{uv}=\va_{uv}|\Theta_M)},\forall u\in\gV, \forall v\in\gV,
\end{align}
% Now we involve the attributes in the generative process. Let $C\in\{(\va_i,\va_j)|i\in\gV,j\in\gV\}$ be a random variable indicating the \emph{attribute value combination} of a randomly sampled pair of nodes, which is independent from $\Theta_M$. Note that $C$ instantiated by different node pairs can be the same, as different nodes can have the same attribute values. $P_{o}(E_{uv}=1|C=\va_{uv},\Theta_M)$ is the conditional probability of an edge $(u,v)$ given the corresponding attribute values on the incident nodes and structural parameters $\Theta_M$, where $\va_{uv}=(\va_u, \va_v)$ denotes the \emph{observed} attribute value combination on nodes $u$ and $v$. Based on Bayes' Theorem, we have
% \begin{align}
% \label{eq:bayes}
%     & P_o(E_{uv}=1|C=\va_{uv},\Theta_M)  \\\nonumber
%   =\,& \frac{P_o(C=\va_{uv}|E_{uv}=1,\Theta_M)P_o(E_{uv}=1|\Theta_M)}{P_o(C=\va_{uv}|\Theta_M)} \\\nonumber
%   =\,& P_M(E_{uv}=1|\Theta_M)\frac{P_o(C=\va_{uv}|E_{uv}=1,\Theta_M)}{P_o(C=\va_{uv}|\Theta_M)},\forall u\in\gV, \forall v\in\gV,
% \end{align}
where the prior distribution on $E_{uv}$ is specified by the structural model $\gM$: i.e., $P_o(E_{uv}=1|\Theta_M) = P_M(E_{uv}=1|\Theta_M)$, and the posterior distribution accounts for the influences from the attribute value combinations. Therefore, the edge probabilities used to generate the observed graph with node attributes is a \emph{modification} of those from a structural graph defined by $\gM$ and $\Theta_M$. 
It is important to clarify that the node attributes are given ahead of graph generation. They are the input to the generative process, not the output. Hence, $P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)$ represents the probability that in all edges, a specific attribute value combination $\va_{uv}$ is observed on an edge's incident nodes. It 
is thus the same for all edges whose incident nodes have the same attribute value combination.
% , no matter where they are, since $C_{uv}$ is independent from the graph structure $\Theta_M$. 

% Second, we do not need to include all possible characteristics of a node $u$ in $\va_{u}$, as long as they are not introducing ethical concerns or unwanted biases in downstream tasks. In fact, some characteristics can be treated as node features captured by $\Theta_M$ in $\gM$ when generating the underlying graph. Thus we only need to include attributes in $\va_{u}$ whose effect is related to our debiasing purpose. For instance, $\va_u$ can include not only sensitive attributes that we want to debias but also those correlate with the sensitive attributes.
%whose effects are meant to be explicitly kept from the influence of debiasing the sensitive attribute for better utility. 

To simplify the notation, let us define a function that maps the attribute value combination $\va_{uv}$ to the probability ratio that modifies the structural graph into the observed graph by
\begin{equation*}
    R(\va_{uv}) \coloneqq \frac{P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)}{P_o(C_{uv}=\va_{uv}|\Theta_M)}, \forall u\in\gV, \forall v\in\gV.
\end{equation*}
Thus we can rewrite \eqref{eq:bayes} by 
\begin{equation}
\label{eq:prob-decomp}
    P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M) = P_M(E_{uv}=1|\Theta_M)R(\va_{uv}). 
\end{equation}
In this way, we explicitly model the effect of node attributes by $R(\va_{uv})$, which modifies the structural graph distribution $P_M(E_{uv}=1|\Theta_M)$ for generating the observed graph $\gG$. 

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/uge_illustration.pdf}
    \vspace{-3mm}
    \caption{Illustration of Unbiased Graph Embedding (\UGE). The color of the nodes represents the value of their attributes, and different line styles suggest how the observed edges are influenced by attributes in the generative process.}
    \label{fig:UGE}
    \vspace{-2mm}
\end{figure}
\section{Unbiased Graph Embedding from a Bias-Free Graph}
\label{sec:UGE}
% This process motivates us to uncover an underlying bias-free graph by separating out sensitive attributes and only conditioning on non-sensitive attributes for calculating edge probabilities.
In this section, we describe our proposed methods for learning unbiased node embeddings based on the generative modeling of the effects of sensitive attributes in \Cref{sec:under-graph}. In a nutshell, we aim to get rid of the sensitive attributes and modify the structural edge probabilities by only conditioning on non-sensitive attributes. This gives us the edge probabilities of a bias-free graph, from which we can learn unbiased node embeddings.
We illustrate this principle in \Cref{fig:UGE}. 
Consider a world without the sensitive attributes, and the attribute vector of node $u$ becomes $\tilde\va_u = \va_u[m:]$, which only include non-sensitive attributes in $\va_u$. We denote $\tilde{\gG}=(\gV, \tilde\gE, \tilde\gA)$ as the corresponding new graph generated with $\tilde\va_u, \forall u\in\gV$, and $\tilde\va_{uv}=(\tilde\va_u, \tilde\va_v)$. Therefore, $\tilde\gG$ is a bias-free graph without influence from sensitive attributes. If we can learn node embeddings from $\tilde\gG$ instead of $\gG$, the embeddings are guaranteed to be unbiased with respect to sensitive attributes. Specifically, the edge probabilities 
used for generating $\tilde\gG$ can be written as
\begin{equation}
\label{eq:prob-decomp2}
    P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M) = P_M(E_{uv}=1|\Theta_M)\tilde R(\tilde\va_{uv}), 
\end{equation}
where
\begin{equation}
    \tilde R(\tilde\va_{uv}) \coloneqq \frac{P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M)}{P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|\Theta_M)}, \forall u\in\gV, \forall v\in\gV,
\end{equation}
$\tilde{C}_{uv}\in\{(\tilde\va_i,\tilde\va_j)|i\in\gV,j\in\gV\}$ is the random variable indicating attribute value combinations without sensitive attributes, and $P_{\tilde o}$ indicates the distributions used in generating $\tilde\gG$. We name the class of methods that learn embeddings from $\tilde\gG$ as \UGE, simply for \textbf{U}nbiased \textbf{G}raph \textbf{E}mbedding. 
% We illustrate the principle of \UGE in \Cref{fig:UGE}. 
Next we introduce two instances of \UGE. The first is \UGE-W, which reweighs the per-edge loss such that the total loss is from $\tilde\gG$ in expectation. The second method is \UGE-R, which adds a regularization term to shape the embeddings to satisfy the properties as those directly learned from $\tilde\gG$.

\subsection{Weighting-Based \UGE}
To compose a loss based on $\tilde\gG$, we modify the loss function in \eqref{eq:loss} by reweighing the loss term on each edge as
\begin{equation}
\label{eq:uge-loss}
    \gL_{\UGE-W}(\gG) = \sum_{(u,v)\in\gE} \gL_{edge}(\rs_{\btheta}(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})}.
\end{equation}
The following theorem shows that, in expectation, this new loss is equivalent to the loss for learning node embeddings from $\tilde\gG$.

\begin{theorem}
Given a graph $\gG$, and $\tilde R(\tilde\va_{uv}) / R(\va_{uv}), \forall (u,v)\in\gE$,  $\gL_{\UGE-W}(\gG)$ is an unbiased loss with respect to $\tilde\gG$.
\end{theorem}
\begin{proof} We take expectation over the edge observations in $\gG$ as
\begin{align}
\label{eq:expectation}
    & \E\big[\gL_{\UGE-W}(\gG)\big] \\\nonumber
    =\,& \E\Bigg[\sum_{(u,v)\in\gE} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})}\Bigg] \\\nonumber
    =\,& \E\Bigg[\sum_{u\in\gV, v\in\gV} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})}\cdot E_{uv}\Bigg] \\\nonumber
    =\,& \sum_{u\in\gV, v\in\gV} \gL_{edge}(\rs(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})} \cdot P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M) \\\nonumber  
    *=\,& \sum_{u\in\gV, v\in\gV} \gL_{edge}(\rs(\vz_u, \vz_v))\cdot P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M) \\\nonumber
    =\,& \E\Bigg[\sum_{(u,v)\in\tilde\gE} \gL_{edge}(\rs(\vz_u, \vz_v))\Bigg].
\end{align}
The step marked by $*$ uses \eqref{eq:prob-decomp} and \eqref{eq:prob-decomp2}.
\end{proof}
%Therefore, we show that \eqref{eq:uge-loss} is an unbiased loss on the new graph $\tilde\gG$. Since \UGE-W is learning node embeddings from a graph where no sensitive attribute is present, it is sufficient for the embeddings to be unbiased. 
\UGE-W is closely related to the idea of importance sampling \cite{kloek1978bayesian}, which analyzes the edge distribution of the bias-free graph $\tilde\gG$ by observations from the given graph $\gG$. The only thing needed for deploying \UGE-W in existing graph embedding methods is to calculate the weights $\tilde R(\tilde\va_{uv})/R(\va_{uv})$. 
To estimate $R(\va_{uv})$, we need the estimates of $P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M)$ and $P_o(C_{uv}=\va_{uv}|\Theta_M)$. With maximum likelihood estimates on the observed graph, we have 
\begin{align}
\label{eq:estimate-R}
    P_o(C_{uv}=\va_{uv}|E_{uv}=1,\Theta_M) &\approx \frac{\sum_{(i,j)\in\gE}\sI[\va_{ij}=\va_{uv}]}{|\gE|}, \\
    P_o(C_{uv}=\va_{uv}|\Theta_M) &\approx \frac{\sum_{i\in\gV,j\in\gV}\sI[\va_{ij}=\va_{uv}]}{N^2}.
\end{align}
Similarly we can estimate $\tilde R(\tilde \va_{uv})$ by
\begin{align}
    P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M) &\approx \frac{\sum_{(i,j)\in\tilde\gE}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{|\tilde\gE|}, \\\label{eq:estimate-tildeR}
    P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|\Theta_M) &\approx \frac{\sum_{i\in\gV,j\in\gV}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{N^2}.
\end{align}
Note that the estimation of $P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M)$ is based on $\tilde\gE$, which is unfortunately from the implicit bias-free graph $\tilde\gG$ and unobservable. But we can approximate it with $\gE$ in the following way: after grouping node pairs by non-sensitive attribute value combinations $\tilde\va_{uv}$, the sensitive attributes only re-route the edges but do not change the number of edges in each group. Thus,
\begin{align}
    P_{\tilde o}(\tilde{C}_{uv}=\tilde\va_{uv}|E_{uv}=1,\Theta_M) &\approx \frac{\sum_{(i,j)\in\tilde\gE}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{|\tilde\gE|} \\\nonumber
    &= \frac{\sum_{i\in\gV,j\in\gV,\tilde\va_{ij}=\tilde\va_{uv}}\sI[(i,j)\in\tilde\gE]}{|\tilde\gE|} \\\nonumber
    &= \frac{\sum_{i\in\gV,j\in\gV,\tilde\va_{ij}=\tilde\va_{uv}}\sI[(i,j)\in\gE]}{|\tilde\gE|} \\\nonumber
    &= \frac{\sum_{(i,j)\in\gE}\sI[\tilde\va_{ij}=\tilde\va_{uv}]}{|\gE|}.
\end{align}

For node pairs with the same attribute value combination, \eqref{eq:estimate-R}-\eqref{eq:estimate-tildeR} only need to be calculated once instead of for each pair. This can be done by first grouping node pairs by their attribute value combinations and then perform estimation in each group. However, when there are many attributes or attributes can take many unique values, the estimates may become inaccurate since there will be many groups and each group may only have a few nodes. In this case, we can make independence assumptions among the attributes. 
For example, by assuming they are independent, the estimate for a specific attribute value combination over all the $K$ attributes becomes the product of $K$ estimates, one for each attribute. The non-sensitive attributes can be safely removed under this assumption with $\tilde R(\tilde\va_{uv})=1$, and only $R(\va_{uv})$ needs to be estimated as $R(\va_{uv})=\prod_{i=1}^m R(\va_{uv}[i])$.
% the assumption in estimating $\tilde R(\tilde \va_{uv})$; we may need to assume \Theta_M does not influence attribute combinations
% independence assumption when there are many attributes
% extend to other models for estimating the weights; take perspectives from social influence and homophily for estimating the probabilities
Since \UGE-W only assigns pre-computed weights to the loss, the optimization based on it will not increase the complexity of any graph embedding method. 
% The estimation of $R(\va_{uv})$ and $\tilde R(\tilde\va_{uv})$ in \eqref{eq:estimate-R} - \eqref{eq:estimate-tildeR} can be done in groups of attribute value combinations. But when there are many attributes or attributes can take many unique values, the estimates may become inaccurate since there will be many groups and each group might only have a few nodes. In this case, we can make further independence assumptions among the attributes. For example, by assuming they are independent, the estimate for attribute combinations becomes the product of estimates for each attribute. Besides, the non-sensitive attributes can be directly removed under this assumption with $\tilde R(\tilde\va_{uv})=1$, and only $R(\va_{uv})$ needs to be estimated as $R(\va_{uv})=\prod_{i=1}^m R(\va_{uv}[i])$.

\subsection{Regularization-Based \UGE}
We propose an alternative way for \UGE which adds a regularization term to the loss function that pushes the embeddings to satisfy properties required by the bias-free graph $\tilde\gG$. Specifically, when the node embeddings are learned from $\tilde\gG$, their produced edge distributions should be the same with and without the sensitive attributes. To enforce this condition, we need to regularize the discrepancy between $P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ and $P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M)$ induced from the node embeddings. We can use the scores in $\rs_{\btheta}(\vz_u, \vz_v)$ as a proxy to represent edge probability produced by the embeddings of nodes $u$ and $v$, i.e., high $\rs_{\btheta}(\vz_u, \vz_v)$ indicates high probability of an edge between $u$ and $v$. 
%Since the probability $P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ of an edge conditioned on the node attribute value combination $\va_{uv}$ is the same for node pairs with the same attribute value combinations, we can estimate it by
We can measure $P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$ by aggregating node pairs with the same attribute value combination to marginalize out the effect of $\Theta_M$ and focus on the influence from attributes as
\begin{equation}
     Q_{\va_{uv}} = \frac{1}{N_{\va_{uv}}}\sum_{i\in\gV,j\in\gV,\va_{ij}=\va_{uv}}\rs_{\btheta}(\vz_i, \vz_j),
\end{equation}
where we use $Q_{\va_{uv}}$ to denote the approximated measure of $P_o(E_{uv}=1|C_{uv}=\va_{uv},\Theta_M)$, and $N_{\va_{uv}}$ is the number of node pairs that has the attribute value combination $\va_{uv}$. For pairs with the same attribute value combination, $Q_{\va_{uv}}$ only needs to be calculated once. Similarly, $P_{\tilde o}(E_{uv}=1|\tilde{C}_{uv}=\tilde\va_{uv},\Theta_M)$ can be represented by $Q_{\tilde\va_{uv}}$, which can be obtained by aggregating the scores over pairs with non-sensitive attribute value combination $\tilde\va_{uv}$.
%, where $\tilde\va_{uv}$ is the same attribute value combination as $\va_{uv}$ with the sensitive attributes removed. 
Finally, we use $\ell_2$ distance between $Q_{\va_{uv}}$ and $Q_{\tilde\va_{uv}}$ as the regularization
\begin{align}
\label{eq:uge-r}
    &\gL_{\UGE-R}(\gG) \\\nonumber
    =&\; \sum_{(u,v)\in\gE} \gL_{edge}(\rs_{\btheta}(\vz_u, \vz_v)) + \lambda\sum_{u\in\gV, v\in\gV}\norm{Q_{\va_{uv}} - Q_{\tilde\va_{uv}}}_2,
\end{align}
where $\lambda$ controls the trade-off between the per-edge losses and the regularization.

In contrast to adversarial regularizations employed in prior work \cite{madras2018learning,bose2019compositional,agarwal2021towards, dai2021say}, \UGE-R takes a different perspective in regularizing the discrepancy between graphs with and without sensitive attributes induced from the embeddings. All previous regularization-based methods impose the constraint on individual edges. 
We should note that the regularization term is summed over all node pairs, which has a complexity of $O(N^3)$ and can be costly to calculate. But in practice, we can add the regulariztaion by only sampling  batches of node pairs in each iteration during model update, and use $\lambda$ to compensate the strength of the regularization.
% \footnote{Empirically, M group pairs uniformly at random in each round, where M is around 10\% of the number of node groups, can already yield promising results.}

\subsection{Combined Method}
\label{sec:discuss-uge}
% relation to importance sampling, observational study, unbiased l2r
% \UGE-W is related to the idea of importance sampling \cite{kloek1978bayesian}, which analyzes a particular distribution from the samples of a different distribution that is easy to sample from. In unbiased graph embedding, we aim to analyze the underlying graph $\tilde\gG$ by observations from the given graph $\gG$. Since \UGE-W only adds weights to the per-edge loss, the optimization based on it will not increase the complexity of any graph embedding method. The estimation of $R(\va_{uv})$ and $\tilde R(\tilde\va_{uv})$ in \eqref{eq:estimate-R} - \eqref{eq:estimate-tildeR} can be done in groups of attribute value combinations. But when there are many attributes or attributes can take many unique values, the estimates may become inaccurate since there will be many groups and each group might only have a few nodes. In this case, we can make further independence assumptions among the attributes. For example, by assuming they are independent, the estimate for attribute combinations becomes the product of estimates for each attribute. Besides, the non-sensitive attributes can be directly removed under this assumption with $\tilde R(\tilde\va_{uv})=1$, and only $R(\va_{uv})$ needs to be estimated as $R(\va_{uv})=\prod_{i=1}^m R(\va_{uv}[i])$.

% In contrast to adversarial regularizers employed in prior work \cite{madras2018learning,bose2019compositional,agarwal2021towards, dai2021say}, \UGE-R takes a different perspective in regularizing the discrepancy between graphs with and without sensitive attributes produced by the embeddings, as it is based on the concept of underlying unbiased structural graph. All previous regularization-based methods impose the constraint on single edges. 
% We should note the regularization term is summed over all node pairs, which has a complexity of $O(N^3)$ and can be costly to optimize. But in practice, we can add the regulariztaion by only sampling node pairs in each iteration during model update, and use $\lambda$ to compensate the strength of the regularization.

As hinted in \cref{sec:intro}, \UGE-W is a sufficient condition for unbiased graph embedding, since it directly learns node embeddings from a bias-free graph. \UGE-R is a necessary condition, as it requires the learned embeddings to satisfy the properties of a bias-free graph. We can combine them to trade-off the debiasing effect and utility,
\begin{align}
    &\gL_{\UGE-C}(\gG) \\\nonumber
    =&\; \sum_{(u,v)\in\gE} \gL_{edge}(\rs_{\btheta}(\vz_u, \vz_v))\frac{\tilde R(\tilde\va_{uv})}{R(\va_{uv})} + \lambda\sum_{u\in\gV, v\in\gV}\norm{Q_{\va_{uv}} - Q_{\tilde\va_{uv}}}_2,
\end{align}
where we use $\gL_{\UGE-C}(\gG)$ to represent the combined method.
$\gL_{\UGE-C}(\gG)$ thus can leverage the advantages of both \UGE-W and \UGE-R to achieve better trade-offs between the unbiasedness and the utility of node embeddings in downstream tasks. 

